Computer-aided abnormality detection in chest radiographs in a clinical setting via domain-adaptation

Deep learning (DL) models are being deployed at medical centers to aid radiologists for diagnosis of lung conditions from chest radiographs. Such models are often trained on a large volume of publicly available labeled radiographs. These pre-trained DL models' ability to generalize in clinical settings is poor because of the changes in data distributions between publicly available and privately held radiographs. In chest radiographs, the heterogeneity in distributions arises from the diverse conditions in X-ray equipment and their configurations used for generating the images. In the machine learning community, the challenges posed by the heterogeneity in the data generation source is known as domain shift, which is a mode shift in the generative model. In this work, we introduce a domain-shift detection and removal method to overcome this problem. Our experimental results show the proposed method's effectiveness in deploying a pre-trained DL model for abnormality detection in chest radiographs in a clinical setting.

==> tex/experiments.tex <==
1. Cross-validation errors for the classification task
2. Similar to DTN paper, Use samples of all class in source domain and
use samples of all except one class in target domain. Visualize the generated
samples from the target domain.
3.


==> tex/fig-alignflow.tex <==
%
\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{figs/alignflow.pdf}
\caption{Domain shift augmentation by Alignflow}
\end{figure}


==> tex/fig-chestxray14-cam-images.tex <==
%
\begin{figure*}[!h]
\centering
\begin{subfigure}{0.47\textwidth}
\includegraphics[width=0.45\textwidth]{figs/00000001_002_real_B.png}
\includegraphics[width=0.45\textwidth]{example-image-a}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
\includegraphics[width=0.45\textwidth]{figs/00000001_002_fake_A.png}
\includegraphics[width=0.45\textwidth]{example-image-a}
\end{subfigure}
%
\begin{subfigure}{0.47\textwidth}
\includegraphics[width=0.45\textwidth]{figs/00000104_001_real_B.png}
\includegraphics[width=0.45\textwidth]{example-image-a}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
\includegraphics[width=0.45\textwidth]{figs/00000104_001_fake_A.png}
\includegraphics[width=0.45\textwidth]{example-image-a}
\end{subfigure}
%
%\begin{subfigure}{0.47\textwidth}
%\includegraphics[width=0.45\textwidth]{figs/00000035_001_real_B.png}
%\includegraphics[width=0.45\textwidth]{example-image-a}
%\end{subfigure}
%\begin{subfigure}{0.45\textwidth}
%\includegraphics[width=0.45\textwidth]{figs/00000035_001_fake_A.png}
%\includegraphics[width=0.45\textwidth]{example-image-a}
%\end{subfigure}
%
%
\caption{
Style transfer between Chestxray14 and MIMIC-CXR datasets using
CycleGAN.}
\label{fig:cxr-cyclegan-images}
\end{figure*}


==> tex/fig-cxr-cyclegan-images.tex <==
%
\begin{figure*}
\centering
%\includegraphics[width=0.3\textwidth]{figs/cxr_cyclegan_images_label.pdf}
%\includegraphics[width=0.9\textwidth]{figs/cxr_cyclegan_images.jpg}
%\includegraphics[width=0.9\textwidth]{figs/cxr_cyclegan_images_s2.jpg}
\begin{subfigure}{0.47\textwidth}
\includegraphics[width=0.45\textwidth]{figs/00000001_002_real_B.png}
\includegraphics[width=0.45\textwidth]{figs/00000001_002_fake_A.png}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
\includegraphics[width=0.45\textwidth]{figs/00000001_002_real_A.png}
\includegraphics[width=0.45\textwidth]{figs/00000001_002_fake_B.png}
\end{subfigure}
%
\begin{subfigure}{0.47\textwidth}
\includegraphics[width=0.45\textwidth]{figs/00000104_001_real_B.png}
\includegraphics[width=0.45\textwidth]{figs/00000104_001_fake_A.png}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
\includegraphics[width=0.45\textwidth]{figs/00000104_001_real_A.png}
\includegraphics[width=0.45\textwidth]{figs/00000104_001_fake_B.png}
\end{subfigure}
%
\begin{subfigure}{0.47\textwidth}
\includegraphics[width=0.45\textwidth]{figs/00000035_001_real_B.png}
\includegraphics[width=0.45\textwidth]{figs/00000035_001_fake_A.png}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
\includegraphics[width=0.45\textwidth]{figs/00000035_001_real_A.png}
\includegraphics[width=0.45\textwidth]{figs/00000035_001_fake_B.png}
\end{subfigure}
%
%
\caption{
Style transfer between Chestxray14 and MIMIC-CXR datasets using
CycleGAN.}
\label{fig:cxr-cyclegan-images}
\end{figure*}


==> tex/fig-cxr-orig-sc.tex <==
%
\begin{figure}[!tb]
%
\centering
%
\begin{subfigure}{0.23\textwidth}
\centering
\includegraphics[width=0.99\textwidth]{figs/cxr_chestxray_sc_hist2d-noadap.png}
\caption{ChestXray14}
\end{subfigure}
%
\begin{subfigure}{0.23\textwidth}
\centering
\includegraphics[width=0.99\textwidth]{figs/cxr_mimic_sc_hist2d-noadap.png}
\caption{MIMIC-CXR}
\end{subfigure}
%
\caption{
%
Density plot of two PCA modes of wavelet scattering coefficients (WSCs) of two datasets are displayed.
The WSCs are computed using Scattering2D implementation from Kymatio package with parameter setting 
$J=4$, $L=8$, $maxorder=2$ while keep other parameters to default values.
We summed the scattering coefficients over the image domain to obtain translational invarient features.
%
We whitened the WSCs before extracting two PCA components.
}
\label{fig:cxr-orig-sc}
\end{figure}


==> tex/fig-domain-shift-detection.tex <==
%
\begin{figure*}
%
\centering
%
\begin{subfigure}{0.48\textwidth}
\includegraphics[width=0.9\textwidth]{figs/chestxray-scattering-comparison.png}
\caption{Wavelet scattering coefficients}
\label{fig:domain-shift-samples}
\end{subfigure}
%
\begin{subfigure}{0.48\textwidth}
\includegraphics[width=0.9\textwidth]{figs/hypothesis_testing_chestxray14_mimiccxr.png}
\caption{B-test statistics}
\label{fig:domain-shift-btest}
\end{subfigure}
%
\caption{(a) Domain-shift between the samples of MIMIC-CXR and ChestXray14 datasets
is visualized for direct inspection. (b) Maximum mean discrepancy (MMD) estimate 
under the null and alternative hypothesis is plotted (Make it precise).}
%
\label{fig:domain-shift-detection}
\end{figure*}


==> tex/model-arch.tex <==
%
\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{figs/model-arch.pdf}
\caption{Domain shift augmentation model (inspired from LeCun AAAI 2020 talk)}
\end{figure}


==> tex/post-experimental-analysis.tex <==
%


==> tex/resources.tex <==
\begin{enumerate}
\item \url{https://www.kaggle.com/c/prostate-cancer-grade-assessment/overview}
\item \url{https://code-int.ornl.gov/dlq/satellite-imagery-domain-seperation}
\item \url{https://github.com/jfhealthcare/Chexpert}
\item \url{https://code.ornl.gov/ai/imaging/medical/cxr_classification}
\item \url{https://github.com/AMLab-Amsterdam/DIVA}
\item \url{https://github.com/fungtion/DANN}
\item \url{https://github.com/pumpikano/tf-dann}
\item \url{https://pypi.org/project/pytorch-gradcam/}
\item \url{https://github.com/rtqichen/ffjord}
\end{enumerate}

